LMI-based Data-Driven Robust Model Predictive Control

Predictive control, which is based on a model of the system to compute the applied input optimizing the future system behavior, is by now widely used. If the nominal models are not given or are very uncertain, data-driven model predictive control approaches can be employed, where the system model or input is directly obtained from past measured trajectories. Using a data informativity framework and Finsler's lemma, we propose a data-driven robust linear matrix inequality-based model predictive control scheme that considers input and state constraints. Using these data, we formulate the problem as a semi-definite optimization problem, whose solution provides the matrix gain for the linear feedback, while the decisive variables are independent of the length of the measurement data. The designed controller stabilizes the closed-loop system asymptotically and guarantees constraint satisfaction. Numerical examples are conducted to illustrate the method.

==> Sections/Sec1_OLDbackup.tex <==
%Although learning from data is not novel in control engineering, it has become increasingly prevalent over the recent years. 
%There are two key issues with the learning-from-data paradigm that attracts the attention of researchers in the field.
%The first one is how to design control systems directly from data without an intermediate system identification step. 
%The second issue is how to provide theoretical guarantees, e.g. stability and constraints satisfaction, for systems controlled by data-driven approach.

%With regards to the first question and for the scope of linear systems, the fundamental result proposed by \cite{willems2005}, which is often referred as \textit{Willems et al. 's fundamental lemma}, provides an answer on how to replace process model with data. 
%In short, the lemma states that all trajectories of an LTI system can be represented by a finite set of its past trajectories, given that the past trajectories are generated by a sufficiently exciting inputs. This idea has been investigated by .... CITE...., where the stabilizing feedback gain is designed by formulated the problem as LMIs without considering performance and constraints guarantees.

%For constraints satisfaction, a control method that handles hard constraints of inputs and states as well as takes performance criteria into account is model predictive control (MPC). 
%The fundamental idea of MPC is to solve, at each time step, an optimal control problem that predicts the future system behavior based on the current state information. The first part of the resulting optimal trajectory is then applied, and the process is repeated at the next step.
%In conventional approach, MPC requires a model of the plant, which is usually obtained from first principles or measured data via system identification.
%Recently, 
Model predictive control has become a popular control scheme in process control by the ability of efficiently and naturally handling input and states constraint and performance criteria. 
The fundamental idea of MPC is to solve, at each time step, an optimal control problem that predicts the future system behavior based on the current state information. %The first part of the resulting optimal trajectory is then applied, and the process is repeated at the next step.
In conventional approach, MPC requires a model of the plant, which is usually obtained from first principles or measured data via system identification. 
However, model development has been shown to be the most critical and time-consuming step in MPC implementation (\cite{Rossiter2001}) and the performance of MPC critically depends on the quality of the model.
An alternative approach is to design an MPC controller directly from measured data, without prior knowledge of an accurate model, which is often referred as data-driven MPC. The learning-based approach, with the usage of Gaussian process (\cite{Hewing2020}) or Reinforcement Learning (\cite{Zanon2021}), received increasing attention recently. Nevertheless, the drawback of these approach is that they menace the advantage of MPC in handling constraints and provide theoretical guarantees since proving the desirable closed-loop properties is still an open problem.  

With regards to linear time invariant system, the fundamental result proposed by \cite{willems2005}, which is often referred as \textit{Willems et al. 's fundamental lemma}, provides an answer on how to replace process model with data. 
In short, the lemma states that all trajectories of an LTI system can be represented by a finite set of its past trajectories, given that the past trajectories are generated by a sufficiently exciting inputs.
This idea has been investigated by \cite{persis2020}, where the stabilizing feedback gain is designed by formulated the problem as LMIs without considering performance and constraints guarantees.





==> Sections/Sec2_OLDbackup.tex <==
In this section, we revisit the main results in \cite{willems2005} and \cite{persis2020}.

Considering a signal $z:\Z \rightarrow \R^r$, we denote 
\begin{equation*}
    z_{[k,k+T]}=[z(k), ..., z(k+T)]^\top,
\end{equation*}
where $k \in \Z, T \in \N$, and when we denote this signal as $z$, we imply that it is not restricted to any interval.
When we mention about the discrete interval from $k$ to $k+T$, we denote as $[k, k+T]$, instead of $[k, k+T] \cap \Z$, for simplicity.
We denote the Hankel matrix associated to $z$ as
\begin{equation*}
    Z_{i,j,N}=
    \begin{bmatrix}
    z(i) & z(i+1) & \cdots & z(i+N-1)\\
    z(i+1) & z(i+2) & \cdots & z(i+N)\\
    \vdots & \vdots &  \ddots & \vdots\\
    z(i+j-1) & z(i+j) & \cdots & z(i+j+N-2)
    \end{bmatrix},
\end{equation*}
where $i \in \Z$ denotes the time when the first sample of the signal is taken,  $j \in \N$ denotes the number of samples per each column and $N \in \N$ denotes the number of samples per each row. If $j=1$, we simply write as 
\begin{equation*}
    Z_{i,N}=
    \begin{bmatrix}
    z(i) & z(i+1) & \cdots & z(i+N-1)\\
    \end{bmatrix}.
\end{equation*}

We consider a controllable and observable  discrete-time linear system given in the form
\begin{equation}
    x(k+1)=Ax(k)+Bu(k), \label{eq:plant}
\end{equation}
where $x \in \R^n, u \in \R^m$ are the states and control inputs of the system.
In the paper, we use $x_d$, $u_d$ with the subscript $d$ to denote the sample data collected from the system during some experiment.
One fundamental condition that needs to be ensured is that the data $x_d$ and $u_d$ collected from the system has encode all the information for the direct design of the control law, which has been established by \cite{willems2005}.  
First, we need to recall the definition of persistency of excitation.
\begin{defi}
The signal $z_{[0,T-1]} \in \R^r$ is persistently exciting of order L if the matrix
\begin{equation*}
    Z_{0,L,T-L+1}=
    \begin{bmatrix}
    z(0) &  z(1)   &  \cdots  & z(T-L) \\
    z(1) & z(2)     &  \cdots  & z(T-L+1)\\
    \vdots & \vdots &  \ddots & \vdots\\
    z(L-1) & z(L) & \cdots & z(T-1)
    \end{bmatrix}
\end{equation*}
has full rank of $rL$. It should be noted that, a necessary condition for  a signal $z$ to be persistently exciting of order $L$ is that it must be sufficiently long, namely $T\geq(r+1)L-1$.
\end{defi}
The following Lemma is crucial for the data-driven approach that exploits the Willems et al. 's fundamental lemma.
\begin{lem} \label{lemma_pre} (\cite{willems2005,persis2020})
Consider system \eqref{eq:plant}. If the input $ u_{d,[0,T-1]}$ is persistently exciting order $n+t$, then 
\begin{itemize}
    \item \begin{equation}
    \textrm{rank}
    \begin{bmatrix}
    U_{0,t,T-t+1}\\
    \hline
    X_{0,T-t+1}
    \end{bmatrix}= n +tm.
        \end{equation}
    \item there exists $g \in \R^{T-t+1}$ such that
    \begin{equation}
        \begin{bmatrix}
        u_{[0,t-1]}\\
        x_{[0,t-1]}
        \end{bmatrix}=
        \begin{bmatrix}
        U_{0,t,T-t+1}\\
        \hline
        X_{0,t,T-t+1}
    \end{bmatrix} g.
    \end{equation}
\end{itemize}
\end{lem}
Lemma~\ref{lemma_pre} allows us to represent the open-loop and closed-loop  dynamics of system \eqref{eq:plant} by using data from a single past trajectory given that the system is sufficiently excited.
In the following, we only consider the input sequence $u_{d,[0,T-1]}$ of order $t+n$ with $t=1$.%%%%CHECK THIS CONDITION
The only requirement on $T$ is that $T \geq (m+1)n+m$, which is necessary for the persistence of excitation condition to hold. %%%%CHECK THIS CONDITION
From Lemma~\ref{lemma_pre} we have
\begin{equation} \label{eq:rank_cond}
    \textrm{rank}
    \begin{bmatrix}
    U_{0,T}\\
    \hline
    X_{0,T}
    \end{bmatrix}= n +m.
        \end{equation}
If system \eqref{eq:plant} is controlled by a linear state-feedback law 
\begin{equation} \label{eq:u=Kx}
    u=Kx,
\end{equation} 
where $K \in \R^{m \times n}$, by using Lemma~\ref{lemma_pre}, we can derive an equivalent representation of the closed-loop system based on the following lemma.
\begin{lem} (\cite{persis2020}) \label{lemma_persis}
If the condition \eqref{eq:rank_cond} is satisfied, then the closed-loop system of system \eqref{eq:plant} with the linear state-feedback \eqref{eq:u=Kx} has the following representation
\begin{equation} \label{eq:lemma_persis_X1X0}
 x(k+1)=X_{1,T}G_k x(k),
\end{equation}
where $G_k \in \R^{T \times n}$ such that
\begin{equation}
 \begin{bmatrix}\label{eq:KI}
K\\
I
\end{bmatrix}=
\begin{bmatrix}
U_{0,T}\\
\hline
X_{0,T}
\end{bmatrix} G_k,   
\end{equation}
and
\begin{equation}
    u(k)=U_{0,T}G_k x(k).
\end{equation}
\end{lem}
Lemma~\ref{lemma_persis} shows that the controller $K$ can be parametrized with the data collected from a single past trajectory via \eqref{eq:KI}, which means that matrix $G_k$ can be regarded as the decision variable, and we can search for $G_k$ instead of $K$ to guarantee stability and performance specification as long as the condition $I=X_{0,T} G_k$ holds. In this case, $X_{1,T}G_k$ provides an equivalent representation of the closed-loop matrix $A+BK$ with $K=U_{0,T}G_k$. We will use this idea to design an optimal state feedback controller without knowing the matrices $A$ and $B$ of the system satisfying states and input constraints only using past trajectories.



==> Sections/Sec3_OLDbackup.tex <==
In this section, we consider controlling system \eqref{eq:plant} under the constraints $x \in \X$ and $u \in \U$ and the matrices $A$ and $B$ are unknown. 
Instead, the system is persistently exited by the input $u_{d,[0,T-1]}$. To guarantee the condition \eqref{eq:rank_cond}, we need the following assumption on $u_d$ and $T$.
\begin{assumption} \label{assumption_persistent}
The input $u_{d,[0,T-1]}$ for generating data is persistently exciting of order $n+1$.
\end{assumption}
Note that, Assumption~\ref{assumption_persistent} implies that ${T \geq (m+1)n+m}$.
The controller minimizes the infinite horizon cost functional at each sampling time
\begin{equation}\label{eq:cost_FunctionJ}
    J(x(\cdot),u(\cdot))= \sum_k^{\infty}x^\top (k) Q x(k) + u(k)^\top R u(k),
\end{equation}
where $Q \succ 0$ and $ R \succ 0$ are weighting matrices.
The benefit of infinite control laws is that it is shown to guarantee stability.
We need assumptions on the constraints. 
 \begin{assumption}\label{assumption_constraints}
 The constraint sets $\X$ and $\U$ can be described in the form
 \begin{align} \label{eq:constraintslinear}
     \X &= \{x \in \R^{n}: c_{i_x}x \leq 1, i_x=1,..., \bar n\}\\ \nonumber
     \U &= \{u \in \R^{m}: d_{i_u}u \leq 1, i_u=1,..., \bar m\},
 \end{align}
 where $c_{i_x} \in \R^{1 \times n}$ and $d_{i_u} \in \R^{1\times m}$, and $\bar n, \bar m$ are the  numbers of states and inputs constraints, respectively. 
 \end{assumption}
 It should be noted that \eqref{eq:constraintslinear} covers the case where $\X$ and $\U$ are polytopic. 
 Also, \eqref{eq:constraintslinear} can be transformed into
\begin{align}
   \mathcal{W}=\{[x^\top~u^\top]^\top \in \R^{n+m}:c_i x + d_i u \leq 1\}, \label{eq:constraintsetW}
 \end{align}
 where $i=1,...,r$, with $r=\bar n+ \bar m$.
%With the choice of control input as in \eqref{eq:u=Kx}, the set \eqref{eq:constraintsetW} can be written as
%\begin{equation}
%   \mathcal{W}=\{x \in \R^{nx}: w_ix \leq 1, i=1,...,r\}, \label{eq:constraintsetW}
% \end{equation}
% where $w_i=c_i+d_iK$. With this definition, it follows that $\mathcal{W} \subseteq \X$.

We need the following lemma for guaranteeing constraints satisfaction.
 \begin{lem}(\cite{boyd1994}) \label{lemma:eplipsoid}
 An ellipsoid
 \begin{equation} \label{eq:ellipsoidE}
     \mathcal{E}(\alpha)=\{x \in \R^{n}: x^\top P x \leq \alpha\}
 \end{equation}
 is contained in the set $\mathcal{W}=\{x \in \R^{n}: w_ix \leq 1, i=1,...,r\}$ if and only if 
 \begin{equation}
 w_i(\alpha P^{-1}) w_i ^\top \leq 1, i =1,...,r.    
 \end{equation}
\end{lem}
Now, we can state the main results for this section in the following theorems.
\begin{thm}\label{theorem_main1}
Consider the system \eqref{eq:plant}, given that Assumptions~\ref{assumption_persistent} and \ref{assumption_constraints} are satisfied.
If there exist matrices $0 \prec N = N^\top \in \R^{n \times n} $ and  $Y \in \R^{T \times n}$ and a constant $\alpha \in \R^+$ such that 
\begin{equation}\label{eq:theorem_main1}
\begin{cases}
    N=X_{0,T}Y \\
    \begin{bmatrix}
    N \quad& X_{1,T}Y \quad& Y^\top M_d^\top S^{1/2}\\
    Y^\top X^\top_{1,T}  \quad & N \quad & 0 \\
    S^{1/2}M_d Y  \quad & 0 \quad & \alpha I
    \end{bmatrix} > 0 \\
\end{cases}    
\end{equation}
is satisfied, where $S=\textrm{diag}(R,Q)$,   $M_d= \begin{bmatrix}
    U_{0,T}\\
    \hline
    X_{0,T}
    \end{bmatrix}$ 
and ${X_{1,T}=[x_d(1)\quad x_d(2) \quad \cdots \quad x_d(T)]}$. Then, for ${P=\alpha N^{-1}}$ and $K=U_{0,T}YN^{-1}$, the feedback law $u=Kx$ asymptotically stabilize the system \eqref{eq:plant}. Also, $\bar V= x(k)^\top P x(k)$ is the upper bound on the infinite horizon cost functional at time $k$.
\end{thm}
\begin{pf}
\newline
Consider the Lyapunov function $V(k)=x(k)^\top P x(k)$ for the closed-loop system \eqref{eq:plant} with the linear feedback controller \eqref{eq:u=Kx}.  Let consider the condition
\begin{equation} \label{eq:proof_Lyapunov}
    V(k+1)-V(k) < -x^\top (k) Q x(k) - u(k)^\top R u(k)\quad \forall k,
\end{equation}
hold. The idea is to formulate the problem by using the data $\Xd, \Xds,$ and  $\Ud,$´instead of using the model $A$ and $B$.
Therefore, we can use the result \eqref{eq:lemma_persis_X1X0} from Lemma~\ref{lemma_persis} to write the left hand side of \eqref{eq:proof_Lyapunov} as 
\begin{equation*} \label{eq_proof_left}
     V(k+1)-V(k)=x^\top (k) (G_k^\top\Xds^\top P  \Xds G_k-P) x(k).
\end{equation*}
For the right hand side of \eqref{eq:proof_Lyapunov}, we can use \eqref{eq:KI} as follows.
\begin{equation} \label{eq:proof_KI}
    \begin{bmatrix}
    u(k)\\
    x(k)
    \end{bmatrix}=
    \begin{bmatrix}
    K\\
    I
    \end{bmatrix}x(k)=M_d G_k x(k),
\end{equation}
where  $M_d= \begin{bmatrix}
    U_{0,T}\\
    \hline
    X_{0,T}
    \end{bmatrix}$. Hence, the right hand side of \eqref{eq:proof_Lyapunov} is equivalent to
\begin{equation} \label{eq_proof_right}
    -x^\top (k) Q x(k) - u(k)^\top R u(k)=-x^\top (k)G_k^\top M_d^\top S M_d G_k x(k),
\end{equation}
where $S=\textrm{diag}(R,Q)$. Using \eqref{eq_proof_right} and \eqref{eq_proof_left}, \eqref{eq:proof_Lyapunov} is eqivalent to 
\begin{equation} \label{eq:proof_trans1}
    G_k^\top\Xds^\top P \Xds G_k -P+G_k^\top M_d^\top S M_d G_k <0.
\end{equation}
Replacing $P=\alpha N^{-1}$ in \eqref{eq:proof_trans1} with $N=N^\top \succ 0$ and $\alpha >0$; then multiplying $N$ on both left and right of the left hand side of \eqref{eq:proof_trans1} with the change of variable 
\begin{equation}\label{eq:proof_YGkN}
 Y=G_kN,    
\end{equation}
we have
\begin{equation}\label{eq:proof_trans2}
 Y^\top\Xds^\top N^{-1} \Xds Y -N+\alpha^{-1}Y^\top M_d^\top S M_d Y <0.  
\end{equation}
Applying Schur complement on \eqref{eq:proof_trans2}, we obtain the inequality in \eqref{eq:theorem_main1}.
It should be note that, from \eqref{eq:KI} we know that $I=\Xd G_k$. Combining with \eqref{eq:proof_YGkN}, we have $N=\Xd G_k N=\Xd Y$, which is the equality in \eqref{eq:theorem_main1}. Since \eqref{eq:theorem_main1} is satisfied, it means \eqref{eq:proof_Lyapunov} is satisfied, which means the closed-loop system is asymptotically stable. 

If we sum both side of \eqref{eq:proof_Lyapunov} from $k$ to $\infty$, we have
\begin{equation*}
    V(\infty)-V(k) < - \sum_k^{\infty}(x^\top (k) Q x(k) + u(k)^\top R u(k)).
\end{equation*}
Since the closed-loop system is asymptotically stable,\\${V(\infty) \rightarrow 0}$, therefore $J(x,u) < V(k)$.\hfill $\blacksquare$
\end{pf}

Theorem~\ref{theorem_main1} provides sufficient conditions to guarantee stability of closed-loop system and an upper bound of the infinite cost, but so far no constraints satisfaction has been guaranteed. The following can be used to compute the linear feedback gain $K$ for a given state $x(k)$ of the closed-loop system to minimize the infinite cost function and satisfy input and state constraints.
\begin{thm}\label{eq:theorem_main2}
Let $x(k)$ be the state of the system \eqref{eq:plant} and given that Assumptions~\ref{assumption_persistent} and \ref{assumption_constraints} are satisfied.
The controller \eqref{eq:u=Kx} obtained by solving the optimization problem
\begin{subequations} \label{eq:opt_prob}
	\begin{align}
	\min_{0 \prec N= N^\top \in \R^{n \times n},Y\in \R^{T \times n},\alpha >0}  ~\alpha  \quad    & \\
	\intertext{subject to}
	\begin{bmatrix} \label{eq:theorem2_ellip}
    1 & x^\top (k)\\ 
    x(k)& N
    \end{bmatrix} & > 0, \\\label{eq:theorem2_stab1}
    N= X_{0,T} & Y,\\ 
    \begin{bmatrix} \label{eq:theorem2_stab2}
    N \quad& X_{1,T}Y \quad& Y^\top M_d^\top S^{1/2}\\
    Y^\top X^\top_{1,T}  \quad & N \quad & 0 \\
    S^{1/2}M_d Y  \quad & 0 \quad & \alpha I
    \end{bmatrix} & > 0, \\
     %
     \begin{bmatrix} \label{eq:theorem2_constraints}
      1    &    [d_i\quad c_i]M_d Y\\
      Y^\top M_d^\top [d_i\quad c_i]^\top  &     N
     \end{bmatrix}  & \geq 0,\\ \nonumber
     i=1,...,& r,
	\end{align}
\end{subequations}
where $K=U_{0,T}YN^{-1}$ and ${P=\alpha N^{-1}}$, asymptotically stabilizes the closed-loop system and the input and states constraints \eqref{eq:constraintslinear} are satisfied. Also, $\alpha$ is the upper bound on the infinite horizon cost functional at time $k$.
\end{thm}
\begin{pf}\\
Clearly, by using \eqref{eq:theorem2_stab1} and \eqref{eq:theorem2_stab2}, the stability of the closed-loop and the upper bound of the cost function are directly derived from Theorem~\ref{theorem_main1}.
The constraints satisfaction is proved by applying Lemma~\ref{lemma:eplipsoid}.
With the choice of control input as in \eqref{eq:u=Kx} and by using \eqref{eq:proof_KI}, the set \eqref{eq:constraintsetW} can be written as
\begin{equation}
 \bar{\mathcal{W}}=\{x \in \R^n: w_ix \leq 1, i=1,...,r\}, \label{eq:constraintsetW}
 \end{equation}
where $w_i=[d_i\quad c_i]M_d G_k$. Obviously, $\bar{\mathcal{W}} \subseteq \mathcal{W}$.
Applying Schur compliment on \eqref{eq:theorem2_ellip}, we have 
\begin{equation} \label{eq:proof2_alp}
    1-\alpha^{-1}x^\top (k) P x(k) >0,~\textrm{or}~V(k)=x^\top (k) P x(k) < \alpha.
\end{equation}
In order satisfy the constraints, we want the ellipsoid $x^\top P x \leq \alpha$ to stay inside  $\bar{\mathcal{W}}$, which means
 \begin{equation*}
 w_i(\alpha P^{-1}) w_i ^\top \leq 1, i =1,...,r,    
 \end{equation*}
where $w_i=[d_i\quad c_i]M_d G_k$. Using Schur compliment and ${P=\alpha N^{-1}}$, we can obtain \eqref{eq:theorem2_constraints}.
From Theorem~\ref{theorem_main1} and \eqref{eq:proof2_alp}, it shows that the cost function $J < V(k) <\alpha$, so $\alpha$ is the upper bound of the infinite cost function $J$.\hfill $\blacksquare$
\end{pf}


==> Sections/Sec4_OLDbackup.tex <==
\subsection{Slowly varying systems}
In this section, we consider the polytopic plant described by
\begin{equation}\label{eq:plant_robust}
    x(k+1)=\Aj x(k)+\Bj u(k), \quad [\Aj~ \Bj] \in \Omega, 
\end{equation}
where the set $\Omega$ is a polytope 
\begin{equation} \label{eq:convexhull}
    \Omega= \textrm{Co}\{[A_1~B_1], [A_2~B_2], ..., [A_\eta~B_\eta]\},
\end{equation}
and $\textrm{Co}$ refers to the convex hull.
In other words, if $[A\quad B] \in \Omega$, then for some $\lambda_j>0$ such that $\sum_{j=1}^{\eta} \lambda_j=1$, we have 
\begin{equation*}
    [A~B]=\sum_{j=1}^{\eta} \lambda_i[\Aj~\Bj].
\end{equation*}
Polytopic system can be used to approximate systems working in different operating points, linear time-varying systems, linear systems with multiplicative uncertainty and nonlinear systems whose the Jacobian lies inside the polytope $\Omega$ in \eqref{eq:convexhull} (\cite{KOTHARE1996}).
For the case of systems with different operating points and each (unknown) pair $[\Aj~\Bj]$ is the model of the system at each operating point, we can apply the method proposed in Section~\ref{sec3} at each operating point: we excite the plant with a sufficient persistently exciting signal and collect the data set $x_{d[0,T]}\tj, u_{d[0,T-1]}\tj$; then by using Theorem~\ref{eq:theorem_main2}, we can obtain $K\tj$ such that $u=K\tj x$ stabilizes the plant at each operating point.
For uncertain linear systems or (slowly) varying systems, we may need to design a robust control law $u=Kx$ to stabilize the system as long as  $[A\quad B] \in \Omega$. 
However, since we do not know the vertices of the polytope $\Omega$, we need to assume that we are able to collect data that can provide us the information of them.
\begin{assumption}\label{assumption_const}
During the time $T$ when the system is persistently excited, the matrices $\Aj$ and $\Bj$ remains constant.
\end{assumption}
This assumption is applicable for slowly varying linear systems.
For each vertex $j$, we assume that by using the same test input $u_{d[0,T-1]}$ which is designed to be sufficient excitation, we collect the data set $x_{d[0,T]}\tj$, then the result from \eqref{theorem_main1} can be naturally extended to the case of system \eqref{eq:plant_robust} as follows.
%%%%%%%
\begin{thm}\label{theorem_main1_robust}
Consider the system \eqref{eq:plant_robust}, given that Assumptions~\ref{assumption_persistent}, \ref{assumption_constraints} and \ref{assumption_const} are satisfied.
If there exist matrices $0 \prec N = N^\top \in \R^{n \times n} $ and  $Y \in \R^{T \times n}$ and a constant $\alpha \in \R^+$ such that 
\begin{equation}\label{eq:theorem_main1_robust}
\begin{cases}
    N=X^{(j)}_{0,T}Y \\
    \begin{bmatrix}
    N \quad& X^{(j)}_{1,T}Y \quad& Y^\top M_d^{(j)\top} S^{1/2}\\
    Y^\top X^{(j)\top}_{1,T}  \quad & N \quad & 0 \\
    S^{1/2}M_d^{(j)} Y  \quad & 0 \quad & \alpha I
    \end{bmatrix} > 0 \\
\end{cases}    
\end{equation}
is satisfied, where $S=\textrm{diag}(R,Q)$,   $M_d^{(j)}= \begin{bmatrix}
    U^{(j)}_{0,T}\\
    \hline
    X^{(j)}_{0,T}
    \end{bmatrix}$ 
and ${X^{(j)}_{1,T}=[x^{(j)}_d(1)\quad x^{(j)}_d(2) \quad \cdots \quad x^{(j)}_d(T)]}$. Then, for ${P=\alpha N^{-1}}$ and $K=U_{0,T}YN^{-1}$, the feedback law $u=Kx$ asymptotically stabilize the system \eqref{eq:plant}. Also, $\bar V= x(k)^\top P x(k)$ is the upper bound on the infinite horizon cost functional at time $k$.
\end{thm}
%%%%%%%%
\begin{pf}
The proof is similar to that of Theorem~\ref{theorem_main1}. The only different is the condition \eqref{eq:proof_Lyapunov} needs to be held for all the vertex of the polytope \eqref{eq:convexhull}. Since $\Omega$ is convex, when the conditions \eqref{eq:theorem_main1_robust} hold for all the vertices, they hold for all $[A\quad B] \in \Omega$, (see \cite{boyd1994}, \cite{KOTHARE1996}).\hfill $\blacksquare$
\end{pf}
There are several points we need discuss with the results from Theorem~\ref{theorem_main1_robust}. First,
as can be seen from the way we compute the gain $K=U_{0,T}YN^{-1}$, we need to use the same test input $u_{d[0,T-1]}$ for all the time we collect data so that we can obtain a single $K$ that robustly stabilize the closed-loop.  
Second, two matrices $ N = N^\top \in \R^{n \times n} $ and  $Y \in \R^{T \times n}$ have $\dfrac{n(n+1)}{2}+Tn$ variables, while $N=X^{(j)}_{0,T}Y$ has $\eta n$ equations. Therefore, a necessary condition for \eqref{eq:theorem_main1_robust} to be feasible is $T>\eta -\dfrac{n+1}{2}$. If this condition is not held, one may consider increase the length $T$ of the test input.

In the robust case, we propose to calculate the matrix gain $K$ repeatedly at each time $k$, as presented in the following Theorem.
%%%%%%%%
\begin{thm}\label{eq:theorem_main3}
Let $x(k)$ be the state of the system \eqref{eq:plant} and given that Assumptions~\ref{assumption_persistent} and \ref{assumption_constraints} are satisfied.
The controller \eqref{eq:u=Kx} obtained by the repeated solution of the optimization problem
\begin{subequations} \label{eq:opt_prob3}
	\begin{align}
	\min_{0 \prec N_k= N_k^\top \in \R^{n \times n},Y_k\in \R^{T \times n},\alpha_k >0}  ~\alpha_k  \quad    & \\
	\intertext{subject to}
	\begin{bmatrix} \label{eq:theorem3_ellip}
    1 & x^\top (k)\\ 
    x(k)& N_k
    \end{bmatrix} & > 0, \\\label{eq:theorem3_stab1}
    N_k= X_{0,T}^{(j)} & Y_k,\\ 
    \begin{bmatrix} \label{eq:theorem3_stab2}
    N_k \quad& X^{(j)}_{1,T}Y_k \quad& Y_k^\top M_d^{(j)\top} S^{1/2}\\
    Y_k^\top X^{(j)\top}_{1,T}  \quad & N_k \quad & 0 \\
    S^{1/2}M_d^{(j)} Y_k  \quad & 0 \quad & \alpha I
    \end{bmatrix} & > 0, \\
     %
     \begin{bmatrix} \label{eq:theorem3_constraints}
      1    &    [d_i\quad c_i]M_d^{(j)} Y_k\\
      Y_k^\top M_d^{(j)\top} [d_i\quad c_i]^\top  &     N_k
     \end{bmatrix}  & \geq 0,\\ \nonumber
     i=1,..., r,~\textrm{and}&~j=1,..., \eta
	\end{align}
\end{subequations}
where $K_k=U_{0,T}Y_kN_k^{-1}$ and ${P_k=\alpha N_k^{-1}}$, has the following properties:
\begin{enumerate}[label=(\alph*)]
\item \textit{Recursive feasibility}: The optimization problem \eqref{eq:opt_prob3} is feasible at time $k+1$ if it is feasible at time $k$.
\item \textit{Optimality}: The solution of optimization problem \eqref{eq:opt_prob3} minimizes the upper bound $\bar V_k=x^\top (k) P_k x(k)$ on the cost functional \eqref{eq:cost_FunctionJ} at each time $k$.
\item \textit{Asymptotic stability}: If the optimization problem \eqref{eq:opt_prob3} is feasible at time $k=0$, the controller $\eqref{eq:u=Kx}$ asymptotically stabilizes the closed-loop system \eqref{eq:plant_robust} under the constraints \eqref{eq:constraintslinear} for all $k \geq 0$.

\end{enumerate}
\end{thm}
%%%%%%%%
\begin{pf}\\
The proof is divided into 3 parts corresponding to the properties(a),(b), and (c).\\
(a)  Assume that the optimization problem \eqref{eq:opt_prob3} is feasible at time $k$, which means there exist $\alpha_k, N_k, Y_k$ as the solution at time $k$. Consider solving the problem \eqref{eq:opt_prob3} at time $k+1$, to prove that the optimization problem is feasible at $k+1$, we need to show that $\alpha_k, N_k, Y_k$ still satisfy all constraints at $k+1$. Since the constraints \eqref{eq:theorem3_stab1}, \eqref{eq:theorem3_stab2}, \eqref{eq:theorem3_constraints} are the same, obviously they are all satisfied. 
We need to show that \eqref{eq:theorem3_ellip} still holds for $k+1$ as follows.
Since \eqref{eq:theorem3_stab1} and \eqref{eq:theorem3_stab2} hold for all $j$ at time $k$, from Theorem~\ref{theorem_main1_robust} we have 
\begin{equation}\label{eq:theorem3proof_1}
    x^\top (k+1) P_k x(k+1) < x(k)^\top P_k x(k)<\alpha_k,
\end{equation}
Using ${P_k=\alpha N_k^{-1}}$, then \eqref{eq:theorem3proof_1} is equivalent to 
\begin{equation*}
    x^\top(k+1)N_k^{-1}x(k+1) < 1,
\end{equation*}
which means \eqref{eq:theorem3_ellip} still holds. Therefore, the optimization problem \eqref{eq:opt_prob3} is feasible at time $k+1$.\\
(b) It is similar to the proof of Theorem~\ref{theorem_main1} and \ref{eq:theorem_main2}, we have $\bar V_k=x^\top (k) P_k x(k)<\alpha_k$. Therefore, from Theorem~\ref{eq:theorem_main1_robust}, minimizing $\alpha_k$\\ implies minimization of the cost function $J$.\\
(c) Consider the Lyapunov function $\mathcal{V}(k)=x^\top(k)P_kx(k)$. From \eqref{eq:theorem3proof_1} we have $x^\top (k+1) P_k x(k+1) < \mathcal{V}(k)$. Since the optimization problem \eqref{eq:opt_prob3} is feasible at $k+1$, there exists $P_{k+1}$ such that $x^\top (k+1) P_{k+1} x(k+1) \leq x^\top (k+1) P_k x(k+1) $. Hence, $\mathcal{V}(k+1) < \mathcal{V} (k)$, resulting in $\mathcal{V}(k+1) - \mathcal{V} (k)<0$.
Therefore, the closed-loop system is asymptotically stable. 
The constraints satisfaction is similar to the proof of Theorem~\ref{eq:theorem_main2}.
\end{pf}


\subsection{Systems with additive noise}
In this section, we consider a linear system with noise 
\begin{equation}\label{eq:plant_noise}
    x(k+1)=A x(k)+B u(k) + d(k), 
\end{equation}
where $d$ is  a bounded disturbance $d \in \mathcal{W}$ such that
\begin{assumption}\label{assumption_noise}
$\|d(k)\| \leq \bar d$ and $\bar d$ is known.
\end{assumption}
The control task here is to stabilize the system at the origin under the constraints \eqref{eq:constraintslinear} and minimize the cost function \eqref{eq:cost_FunctionJ}. In this case, the data collected from past trajectories is already corrupted with noise.
We use the notion $D$ as the vector of noise 
\begin{align}
    D_{0,T} & =[d(0)\quad d(1)\quad...\quad d(T-1)]\\
    D_{1,T} &=[d(1) \quad d(2)\quad...\quad d(T)].
\end{align}
With the assumption \eqref{assumption_noise}, there exists $R_D$ such that
\begin{equation}
D D^{\top}\leq R_D R_D^\top.    
\end{equation}
We have to guarantee the constraints for the state affected by noise, so we need to guarantee that $x(k) \in \bar{\mathcal{X}}$ where 
$\bar{\mathcal{X}}= \mathcal{X} \ominus \mathcal{W}$
% \begin{assumption}\label{assumption_noise}
% There exists a known $R_D$ such that $D D^{\top}\preceq R_D R_D^\top$.
% \end{assumption}
\begin{thm}\label{eq:theorem_noise}
Let $x(k)$ be the state of the system \eqref{eq:plant} and given that Assumptions~\ref{assumption_persistent} and \ref{assumption_constraints} are satisfied.
The controller \eqref{eq:u=Kx} obtained by solving the optimization problem
\begin{subequations} \label{eq:opt_prob}
	\begin{align}
	\min_{0 \prec N= N^\top \in \R^{n \times n},Y\in \R^{T \times n},\alpha >0}  ~\alpha  \quad    & \\
	\intertext{subject to}
	\begin{bmatrix} \label{eq:theorem3_ellip}
    1 & x^\top (k)\\ 
    x(k)& N
    \end{bmatrix} & > 0, \\\label{eq:theorem3_stab1}
    N= X_{0,T} & Y,\\ 
    \begin{bmatrix} \label{eq:theorem2_stab2}
    N \quad& X_{1,T}Y \quad& Y^\top M_d^\top S^{1/2} \quad & 0\\
    Y^\top X^\top_{1,T}  \quad & N \quad & 0 \quad & Y^\top\\
    S^{1/2}M_d Y  \quad & 0 \quad & \alpha I \quad & 0 \\
    0 \quad & Y \quad & 0 \quad  & \varepsilon_1 I
    \end{bmatrix} & > 0, \\
     %
     \begin{bmatrix} \label{eq:theorem3_constraints}
      1    &    [\bar d_i\quad \bar c_i]M_d Y\\
      Y^\top M_d^\top [\bar d_i\quad \bar c_i]^\top  &     N
     \end{bmatrix}  & \geq 0,\\ \nonumber
     i=1,...,& r,\\
    \begin{bmatrix} \label{eq:theorem3_constraints_plus}
      1 - \varepsilon_2 q_i R_D R_D q_i^\top   &    q_iX_1 Y & 0\\
      Y^\top X_1^\top q_i  &     N   &    Y^\top\\
      0 &  Y^\top&   \varepsilon_2 I
     \end{bmatrix}  & \geq 0,\\ \nonumber
     i=1,...,& \bar r,
	\end{align}
\end{subequations}
where $K=U_{0,T}YN^{-1}$ and ${P=\alpha N^{-1}}$, asymptotically stabilizes the closed-loop system and the input and states constraints \eqref{eq:constraintslinear} are satisfied. Also, $\alpha$ is the upper bound on the infinite horizon cost functional at time $k$.
\end{thm}
\begin{pf}\\
By using the notation from previous proof, we can have
\begin{equation*}
    \Xds=A\Xd+BU_0+D,
\end{equation*}
and hence, the dynamics of the system \eqref{eq:plant_robust} can be written as
\begin{equation} \label{eq:plant_robust_para}
    x(k+1)=(\Xds-D)G_k x + d.
\end{equation}
By using Theorem \ref{theorem_main1}, the condition to stabilize system \eqref{eq:plant_robust_para}  is
\begin{align}
    & N=X_{0,T}Y \\
    & \begin{bmatrix} \label{eq:proof3_ineq}
    N \quad& (X_{1,T}-D)Y \quad & Y^\top M_d^\top S^{1/2}\\
    Y^\top (X_{1,T}-D)^\top  & N \quad & 0 \\
    S^{1/2}M_d Y  \quad & 0 \quad & \alpha I
    \end{bmatrix} > 0 \\ \nonumber
\end{align}
We can use Cauchy–Schwarz inequality in the following form
\begin{equation*}
    MD^\top N + N^\top D M^\top \leq \epsilon M M^\top + \epsilon^{-1} N^\top D D^\top N, \quad \forall M, N.
\end{equation*}
Since we have $D D^{\top}\leq R_D R_D^\top$, the inequality above can be written as
\begin{equation} \label{eq:proof3_ineq2}
    MD^\top N + N^\top D M^\top \leq \epsilon M M^\top + \epsilon^{-1} N^\top R_D R_D^\top N, \quad \forall M, N.
\end{equation}
Applying \eqref{eq:proof3_ineq2} as follows,
\begin{equation*}
    \begin{bmatrix}
    0 & DY & 0\\
    Y^\top D^\top & 0 & 0 \\
    0 & 0 & 0
    \end{bmatrix} \leq \varepsilon_1^{-1} \begin{bmatrix}
    0\\
    Y^\top \\
    0
    \end{bmatrix}
    \begin{bmatrix}
    0 & Y & 0 \\
    \end{bmatrix} + \varepsilon \begin{bmatrix}
    I\\
    0 \\
    0\\
    \end{bmatrix}R_D R_D^\top
    \begin{bmatrix}
    I & 0 & 0
    \end{bmatrix},
\end{equation*}
and then applying to \eqref{eq:proof3_ineq2}, we obtain \eqref{eq:theorem2_stab2}.
Condition \eqref{eq:theorem3_constraints} is for constraints guaranteeing, which are similar to that of previous Theorems, except that the constants are now different because now we need to guarantee the states staying inside set $\bar{\mathcal{X}}$ instead of $\mathcal{X}$ due to disturbance.
Condition  \eqref{eq:theorem3_constraints_plus} is for guaranteeing constraints of $x(k+1)$. This condition does not appear in previous Theorems because without the disturbance, the Lyapunov function reduces in each $k$ means that $\|x(k+1)\| < \|x(k)\|$. However, for this case, the reduction of Lyapunov function only guarantee for nominal system. In order to make sure the state $x(k+1)$ also stays in the bounds under disturbance, we need to make sure $x(k+1) \in \bar{\mathcal{X}}$. 
In order to do this, we need to make sure the ellipsoid corresponding to the state $x(k+1)$ is also contained in the polytope.  
\end{pf}

